Performance Prediction for Coarse-Grained Locking

A standard design pattern found in many concurrent data structures, such as hash tables or ordered containers, is an alternation of parallelizable sections that incur no data conflicts and critical sections that must run sequentially and are protected with locks. A lock can be viewed as a queue that arbitrates the order in which the critical sections are executed, and a natural question is whether we can use stochastic analysis to predict the resulting throughput. As a preliminary evidence to the affirmative, we describe a simple model that can be used to predict the throughput of coarse-grained lock-based algorithms. We show that our model works well for CLH lock, and we expect it to work for other popular lock designs such as TTAS, MCS, etc.

==> pics/execution-main.tex <==
\begin{tikzpicture}

\node at (-3.8,0.6) {$1$};
\draw (-3.6,0.6) -- (-3.4,0.6);
\draw (-2.4,0.8) -- (-3.4,0.8) -- (-3.4,0.4) -- (-2.4,0.4);
\node at (-2.9,0.6) {$W/X$};

\draw[fill=blue!10] (-2.4,0.8) -- (-2.4,0.4) -- (0.8,0.4) -- (0.8,0.8) -- cycle;
\draw (-1.6,0.8) -- (-1.6,0.4);
\draw (0.2,0.8) -- (0.2,0.4);
\node at (-2,0.6) {$R_I$};
\node at (-0.7,0.6) {$C$};
\node at (0.5,0.6) {$W$};
\draw [fill=red!10] (10,0.4) -- (0.8,0.4) -- (0.8,0.8) -- (10,0.8);
\draw (1.4,0.8) -- (1.4,0.4);
\draw (9.4,0.8) -- (9.4,0.4);
\node at (1.1,0.6) {$W$};
\node at (5.4,0.6) {$P$};
\node at (9.7,0.6) {$W$};

\node at (-3.8,0) {$2$};
\draw (-3.6,0) -- (-2.4,0);
\draw (-2.4,-0.2) -- (-1.4,-0.2) -- (-1.4,0.2) -- (-2.4,0.2) -- cycle;
\node at (-1.9,0) {$W/X$};
\draw (-1.4,0) -- (0.8,0);
\draw [fill=blue!10] (0.8,0.2) -- (0.8,-0.2) -- (4,-0.2) -- (4,0.2) -- cycle;
\draw (1.6,0.2) -- (1.6,-0.2);
\draw (3.4,0.2) -- (3.4,-0.2);
\node at (1.2,0) {$R_I$};
\node at (2.5,0) {$C$};
\node at (3.7,0) {$W$};
\draw [fill=red!10] (10.6,0.2) -- (4,0.2) -- (4,-0.2) -- (10.6,-0.2);
\draw (4.6,0.2) -- (4.6,-0.2);
\node at (4.3,0) {$W$};
\node at (8.6,0) {$P$};

\node at (-3.8,-1.2) {$N$};
\draw (-3.6,-1.2) -- (-0.4,-1.2);
\draw (-0.4,-1) -- (-0.4,-1.4) -- (0.6,-1.4) -- (0.6,-1) -- cycle;
\node at (0.1,-1.2) {$W/X$};
\draw (0.6,-1.2) -- (7.2,-1.2);
\draw [fill=blue!10] (7.2,-1) -- (7.2,-1.4) -- (10.4,-1.4) -- (10.4,-1) -- cycle;
\draw (8,-1) -- (8,-1.4);
\draw (9.8,-1) -- (9.8,-1.4);
\node at (7.6, -1.2) {$R_I$};
\node at (8.9,-1.2) {$C$};
\node at (10.1,-1.2) {$W$};

\node at (14.6,0) {};

\end{tikzpicture}

==> queue.tex <==
\section{Simplified queue model}
As described in the previous section we try to analyse
coarse-grained algorithms of specific form.
%
We miss one important detail: which lock we use,
but it is not important for our simple analysis.
%
Consider the operation of a data structure
in a therminology of queueing theory:
when a process comes it enters the service, if the server is free,
or it joins a queue, otherwise; the service takes time
exponentially distributed with mean $\mu = \frac{1}{C}$;
upon completing service process departs the system and returns after time
exponentially distributed with mean $\lambda = \frac{1}{P}$.
%
Then, it can be calculated that the average amount of
processes in the system is approximately
equal to $T - \frac{\mu}{\lambda} = T - \frac{P}{C}$.

From that we can calculate the time that takes an execution of the operation
on average.
%
It should be approximately equal to
$\max(T - \frac{P}{C}, 1) \cdot C + P$.
%
Thus, the throughput is equal to $\frac{\alpha \cdot T}{\max(T - \frac{P}{C}, 1) \cdot C + P}$.
%
To clarify a little bit further: if the throughput equals to $\frac{\alpha \cdot T}{C + P}$, if $(T - 1) \cdot C < P$,
or to $\frac{\alpha}{C}$, otherwise.

